The geometry of the Thurston metric: a survey

This paper is a survey about the Thurston metric on the Teichm\"uller space. The central issue is the constructions of extremal Lipschitz maps between hyperbolic surfaces. We review several constructions, including the original work of Thurston. Coarse geometry and isometry rigidity of the Thurston metric, relation between the Thurston metric and the Thurston compactification are discussed. Some recent generalizations and developments of the Thurston metric are sketched.

==> Comparison.tex <==
  \section{Comparison with other metrics}
  
  
  \HP{Since the paper is not posted in arXiv, we just mention this comparison in the introduction.}
  \begin{lemma}[Wolpert, HOPP, Burns-Masur-Wilkinson, McMullen]
  There exists a constant $C$ depending on the topology of $S$ such that for any $X\in\T(S)$ and any $v\in T_X\T(S)$,
  	  \begin{eqnarray*}
  C\cdot\ell_{syst}(X)\|v\|_T\leq &	\|v\|_{Th}&\leq \|v\|_T  \qquad (\textup{HOPP, Wolpert})\\
 C \|v\|_{wp} \leq &\|v\|_{Th}&\leq \frac{C}{\ell_{syst}(X)} \|v\|_{wp} \qquad (\textup{HOPP, Wolpert, Burns-Masur-Wilkinson })\\
  {C}{\ell_{syst}(X)} \|v\|_{T} \leq &\|v\|_{wp}& C\leq  \|v\|_T\qquad (\textup{ Burns-Masur-Wilkinson, McMullen })\\
  &\|v\|_{Th}&\geq C \|v\|_e \qquad (\textup{HOPP})\\
 &\|v\|_{e}&\leq C \|v\|_{wp}  \qquad (\textup{HOPP})\\
 C\|v\|_M\leq &\|v\|_T & \leq  C \|v\|_M
 \qquad (\textup{ McMullen})
  \end{eqnarray*}
  \end{lemma}
  


==> Envelopes.tex <==
\section{Envelopes}
 



==> LengthFunctions.tex <==
\section{Behavior of geodesics (\alert{check the boundary section and the shearing section})}
\subsection{Convexity of Length functions} Recall that every maximal  lamination on $X$ provides a \emph{shearing coordinates} of $\T(S)$.  %In \cite{BBFS2013}, Bestvina, Bromberg, Fujiwara, and Souto proved that the following convexity:
\begin{theorem}[\cite{BBFS2013}, Theorem 1.3]
	Let $S$ be an orientable surface of finite type with negative Euler characteristic. Let $\lambda$  be a maximal lamination in $S$ with finitely many leaves. Then for any essential closed curve $\alpha$, the length function $\ell_\alpha:\T(S)\to\R$ is convex with respect to the shearing coordinates associated to $\lambda$. Moreover, if $\alpha$ intersects all the leaves of $\lambda$ transversely, then $\ell_\alpha$ is strictly convex.
\end{theorem}

In \cite{Theret2014},  Th\'eret improved the above result  as:
\begin{theorem}[\cite{Theret2014}, Theorem 1.1]
Let $S$ be an orientable closed surface  with negative Euler characteristic. Let $\lambda$  be an arbitrary maximal lamination in $S$. Then for any measured lamination  $\alpha$, the length function $\ell_\alpha:\T(S)\to\R$ is convex with respect to the shearing coordinates associated to $\lambda$. Moreover, if $\alpha$ intersects all the leaves of $\lambda$ transversely, then $\ell_\alpha$ is strictly convex.
\end{theorem}

\subsection{Convergence to the Thurston boundary in the forward direction}

  convergence of stretch lines $\PML$ (papadopoulos),  Convergence of any Thurston geodesic ray (Walsh). convergence of anti-stretch lines for special cases (Theret), 





==> Questions.tex <==
\section{Questions}

\begin{question}
	Is the Thurston distance function $C^1$, or even $C^2$? (The Teichm\"uller distance is differentiable by Earle (1977 Duke)  but not $C^{2+\epsilon}$ by Rees (2004PLMS)  )  An analogue of the Gardiner formula? In one direction,  it is possible that  
	\begin{equation*}
		<\left.\frac{d}{dt}d_{Th}(X,\cdot)\right|_Y,v>~~\overset{?}{=} v(\frac{d\ell_\lambda}{\ell_\lambda})
	\end{equation*}
	where $\lambda$ is a measured lamination contained in the maximally stretched lamination from $X$ to $Y$. For the other direction, is it true that
		\begin{equation*}
		<\left.\frac{d}{dt}d_{Th}(\cdot ,Y)\right|_X,v>~~\overset{?}{=} - v (\frac{d\ell_\lambda}{\ell_\lambda}).
	\end{equation*}

\end{question}
